Set-Theoretic Compositionality of Sentence Embeddings

Sentence encoders play a pivotal role in various NLP tasks; hence, an accurate evaluation of their compositional properties is paramount. However, existing evaluation methods predominantly focus on goal task-specific performance. This leaves a significant gap in understanding how well sentence embeddings demonstrate fundamental compositional properties in a task-independent context. Leveraging classical set theory, we address this gap by proposing six criteria based on three core "set-like" compositions/operations: \textit{TextOverlap}, \textit{TextDifference}, and \textit{TextUnion}. We systematically evaluate $7$ classical and $9$ Large Language Model (LLM)-based sentence encoders to assess their alignment with these criteria. Our findings show that SBERT consistently demonstrates set-like compositional properties, surpassing even the latest LLMs. Additionally, we introduce a new dataset of ~$192$K samples designed to facilitate future benchmarking efforts on set-like compositionality of sentence embeddings.

==> Images_Codes/H6_Norm/gpt_norm.tex <==
\begin{figure*}[!t]
    % \vspace{-1mm}
    \centering
    \includesvg[width=
    % 0.7\textwidth
    0.7\textwidth
    ]{Images/H6_Union_Norm/gpt_norm.svg}
    \caption{
    Encoder - GPT3
    }
    \label{fig:h6_gpt_norm}
    % \vspace{-1mm}
\end{figure*}

==> Images_Codes/H6_Norm/laser_norm.tex <==
\begin{figure*}[!t]\small
    % \vspace{-1mm}
    \centering
    \includesvg[width=
    % 0.7\textwidth
    0.7\textwidth
    ]{Images/H6_Union_Norm/lsr_norm.svg}
    \caption{
    Encoder - LASER
    }
    \label{fig:h6_laser_norm}
    % \vspace{-1mm}
\end{figure*}

==> Images_Codes/H6_Norm/llama_norm.tex <==
\begin{figure*}[!t]
    % \vspace{-1mm}
    \centering
    \includesvg[width=
    % 0.7\textwidth
    0.7\textwidth
    ]{Images/H6_Union_Norm/llama2_norm.svg}
    \caption{
    Encoder - LLaMa2
    }
    \label{fig:h6_llama_norm}
    % \vspace{-1mm}
\end{figure*}

==> Images_Codes/H6_Norm/sbert_norm.tex <==
\begin{figure*}[!t]
    % \vspace{-1mm}
    \centering
    \includesvg[width=
    % 0.7\textwidth
    0.7\textwidth
    ]{Images/H6_Union_Norm/sbert_norm.svg}
    \caption{
    Encoder - SBERT
    }
    \label{fig:h6_sbert_norm}
    % \vspace{-1mm}
\end{figure*}

==> Images_Codes/H6_Norm/use_norm.tex <==
\begin{figure*}[!t]
    % \vspace{-1mm}
    \centering
    \includesvg[width=
    % 0.7\textwidth
    0.7\textwidth
    ]{Images/H6_Union_Norm/use_norm.svg}
    \caption{
    Encoder - USE
    }
    \label{fig:h6_use_norm}
    % \vspace{-1mm}
\end{figure*}

==> Images_Codes/Model_Projection_Codes/infersent_projection.tex <==
\begin{figure*}[!t]
    % \vspace{-1mm}
    \centering

    % Overlap
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=1.0\textwidth]{Images/H2_Intersection/infersent_int.svg}
         \caption{TextOverlap: The projection embedding mostly lie in the ``middle'' of the embeddings of the input sentences as described in rubric R2 \ref{para:h2_results}.
         This follows  our expectation shown in figure \ref{fig:projection_expectation}b.
         }
         \label{fig:infersent_overlap}
     \end{subfigure}
     % \hfill
    ~
     % Difference
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
        \includesvg[width=1.0\textwidth]{Images/H5_Difference/infersent_diff.svg}
         \caption{TextDifference: The projection embedding is mostly bounded by a small angle around the embedding of the input sentence $A$ (refer R5 \ref{para:h5_results}).
         This follows  our expectation shown in figure \ref{fig:projection_expectation}a.
         }
         \label{fig:infersent_difference}
     \end{subfigure}
     % \hfill
    ~
    % Union
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=\textwidth]{Images/H6_Union/infersent_union.svg}
         \caption{
         TextUnion: The projection embedding mostly lie in ``middle'' of the input sentence embeddings (refer \ref{para:h6_results}). This follows  our expectation shown in figure \ref{fig:projection_expectation}c-middle.  \\ \hspace{\textwidth}
         }
         \label{fig:infersent_union}
     \end{subfigure}
     % \hfill
     

    \vspace{-1mm}
    \caption{Histogram of the angle between the projection of the overlap embedding (onto the plane of the embeddings of the input sentences $A$ and $B$) and the embedding of sentence $B$. We normalize this angle such that the angle between the embeddings of sentences $A$ and $B$ is consistently 1. For computing the embedding we use \textbf{InferSent} and the results for other encoders are shown in the appendix.}
    \label{fig:infersent_projection}
    % \vspace{-1mm}
\end{figure*}

==> Images_Codes/Model_Projection_Codes/laser_projection.tex <==
\begin{figure*}[!t]
    % \vspace{-1mm}
    \centering

    % Overlap
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=1.0\textwidth]{Images/H2_Intersection/lsr_int.svg}
         \caption{TextOverlap: The projection embedding mostly lie in the ``middle'' of the embeddings of the input sentences as described in rubric R2 \ref{para:h2_results}.
         This follows  our expectation shown in figure \ref{fig:projection_expectation}b.
         }
         \label{fig:laser_overlap}
     \end{subfigure}
     % \hfill
    ~
     % Difference
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
        \includesvg[width=1.0\textwidth]{Images/H5_Difference/lsr_diff.svg}
         \caption{TextDifference: The projection embedding is mostly bounded by a small angle around the embedding of the input sentence $A$ (refer R5 \ref{para:h5_results}).
         This follows  our expectation shown in figure \ref{fig:projection_expectation}a.
         }
         \label{fig:laser_difference}
     \end{subfigure}
     % \hfill
    ~
    % Union
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=\textwidth]{Images/H6_Union/lsr_union.svg}
         \caption{
         TextUnion: The projection embedding mostly lie in ``middle'' of the input sentence embeddings (refer \ref{para:h6_results}). This follows  our expectation shown in figure \ref{fig:projection_expectation}c-middle.  \\ \hspace{\textwidth}
         }
         \label{fig:laser_union}
     \end{subfigure}
     % \hfill
     

    \vspace{-1mm}
    \caption{Histogram of the angle between the projection of the overlap embedding (onto the plane of the embeddings of the input sentences $A$ and $B$) and the embedding of sentence $B$. We normalize this angle such that the angle between the embeddings of sentences $A$ and $B$ is consistently 1. For computing the embedding we use \textbf{LASER} and the results for other encoders are shown in the appendix.}
    \label{fig:laser_projection}
    % \vspace{-1mm}
\end{figure*}

==> Images_Codes/Model_Projection_Codes/llama2_projection.tex <==
\begin{figure*}[!t]
    % \vspace{-1mm}
    \centering

    % Overlap
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=1.0\textwidth]{Images/H2_Intersection/llama2_int.svg}
         \caption{TextOverlap: The projection embedding mostly lie in the ``middle'' of the embeddings of the input sentences as described in rubric R2 \ref{para:h2_results}.
         This follows  our expectation shown in figure \ref{fig:projection_expectation}b.
         }
         \label{fig:llama_overlap}
     \end{subfigure}
     % \hfill
    ~
     % Difference
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
        \includesvg[width=1.0\textwidth]{Images/H5_Difference/llama2_diff.svg}
         \caption{TextDifference: The projection embedding is mostly bounded by a small angle around the embedding of the input sentence $A$ (refer R5 \ref{para:h5_results}).
         This follows  our expectation shown in figure \ref{fig:projection_expectation}a.
         }
         \label{fig:llama_difference}
     \end{subfigure}
     % \hfill
    ~
    % Union
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=\textwidth]{Images/H6_Union/llama2_union.svg}
         \caption{
         TextUnion: The projection embedding mostly lie in ``middle'' of the input sentence embeddings (refer \ref{para:h6_results}). This follows  our expectation shown in figure \ref{fig:projection_expectation}c-middle. \\ \hspace{\textwidth}  
         }
         \label{fig:llama_union}
     \end{subfigure}
     % \hfill
     

    \vspace{-1mm}
    \caption{Histogram of the angle between the projection of the overlap embedding (onto the plane of the embeddings of the input sentences $A$ and $B$) and the embedding of sentence $B$. We normalize this angle such that the angle between the embeddings of sentences $A$ and $B$ is consistently 1. For computing the embedding we use \textbf{LLaMA2} and the results for other encoders are shown in the appendix.}
    \label{fig:llama_projection}
    % \vspace{-1mm}
\end{figure*}

==> Images_Codes/Model_Projection_Codes/llama3_projection.tex <==
\begin{figure*}[!t]
    % \vspace{-1mm}
    \centering

    % Overlap
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=1.0\textwidth]{Images/H2_Intersection/llama3_int.svg}
         \caption{TextOverlap: The projection embedding mostly lie in the ``middle'' of the embeddings of the input sentences as described in rubric R2 \ref{para:h2_results}.
         This follows  our expectation shown in figure \ref{fig:projection_expectation}b.
         }
         \label{fig:llama3_overlap}
     \end{subfigure}
     % \hfill
    ~
     % Difference
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
        \includesvg[width=1.0\textwidth]{Images/H5_Difference/llama3_diff.svg}
         \caption{TextDifference: The projection embedding is mostly bounded by a small angle around the embedding of the input sentence $A$ (refer R5 \ref{para:h5_results}).
         This follows  our expectation shown in figure \ref{fig:projection_expectation}a.
         }
         \label{fig:llama3_difference}
     \end{subfigure}
     % \hfill
    ~
    % Union
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=\textwidth]{Images/H6_Union/llama3_union.svg}
         \caption{
         TextUnion: The projection embedding mostly lie in ``middle'' of the input sentence embeddings (refer \ref{para:h6_results}). This follows  our expectation shown in figure \ref{fig:projection_expectation}c-middle. \\ \hspace{\textwidth}  
         }
         \label{fig:llama3_union}
     \end{subfigure}
     % \hfill
     

    \vspace{-1mm}
    \caption{Histogram of the angle between the projection of the overlap embedding (onto the plane of the embeddings of the input sentences $A$ and $B$) and the embedding of sentence $B$. We normalize this angle such that the angle between the embeddings of sentences $A$ and $B$ is consistently 1. For computing the embedding we use \textbf{LLaMA3} and the results for other encoders are shown in the appendix.}
    \label{fig:llama3_projection}
    % \vspace{-1mm}
\end{figure*}

==> Images_Codes/Model_Projection_Codes/mistral_projection.tex <==
\begin{figure*}[!t]
    % \vspace{-1mm}
    \centering

    % Overlap
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=1.0\textwidth]{Images/H2_Intersection/mistral_int.svg}
         \caption{TextOverlap: The projection embedding mostly lie in the ``middle'' of the embeddings of the input sentences as described in rubric R2 \ref{para:h2_results}.
         This follows  our expectation shown in figure \ref{fig:projection_expectation}b.
         }
         \label{fig:mistral_overlap}
     \end{subfigure}
     % \hfill
    ~
     % Difference
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
        \includesvg[width=1.0\textwidth]{Images/H5_Difference/mistral_diff.svg}
         \caption{TextDifference: The projection embedding is mostly bounded by a small angle around the embedding of the input sentence $A$ (refer R5 \ref{para:h5_results}).
         This follows  our expectation shown in figure \ref{fig:projection_expectation}a.
         }
         \label{fig:mistral_difference}
     \end{subfigure}
     % \hfill
    ~
    % Union
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=\textwidth]{Images/H6_Union/mistral_union.svg}
         \caption{
         TextUnion: The projection embedding mostly lie in ``middle'' of the input sentence embeddings (refer \ref{para:h6_results}). This follows  our expectation shown in figure \ref{fig:projection_expectation}c-middle. \\ \hspace{\textwidth}  
         }
         \label{fig:mistral_union}
     \end{subfigure}
     % \hfill
     

    \vspace{-1mm}
    \caption{Histogram of the angle between the projection of the overlap embedding (onto the plane of the embeddings of the input sentences $A$ and $B$) and the embedding of sentence $B$. We normalize this angle such that the angle between the embeddings of sentences $A$ and $B$ is consistently 1. For computing the embedding we use \textbf{Mistral} and the results for other encoders are shown in the appendix.}
    \label{fig:mistral_projection}
    % \vspace{-1mm}
\end{figure*}

==> Images_Codes/Model_Projection_Codes/mpnet_projection.tex <==
\begin{figure*}[!t]
    % \vspace{-1mm}
    \centering

    % Overlap
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=1.0\textwidth]{Images/H2_Intersection/mpnet_int.svg}
         \caption{TextOverlap: The projection embedding mostly lie in the ``middle'' of the embeddings of the input sentences as described in rubric R2 \ref{para:h2_results}.
         This follows  our expectation shown in figure \ref{fig:projection_expectation}b.
         }
         \label{fig:mpnet_overlap}
     \end{subfigure}
     % \hfill
    ~
     % Difference
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
        \includesvg[width=1.0\textwidth]{Images/H5_Difference/mpnet_diff.svg}
         \caption{TextDifference: The projection embedding is mostly bounded by a small angle around the embedding of the input sentence $A$ (refer R5 \ref{para:h5_results}).
         This follows  our expectation shown in figure \ref{fig:projection_expectation}a.
         }
         \label{fig:mpnet_difference}
     \end{subfigure}
     % \hfill
    ~
    % Union
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=\textwidth]{Images/H6_Union/mpnet_union.svg}
         \caption{
         TextUnion: The projection embedding mostly lie in ``middle'' of the input sentence embeddings (refer \ref{para:h6_results}). This follows  our expectation shown in figure \ref{fig:projection_expectation}c-middle. \\ \hspace{\textwidth}  
         }
         \label{fig:mpnet_union}
     \end{subfigure}
     % \hfill
     

    \vspace{-1mm}
    \caption{Histogram of the angle between the projection of the overlap embedding (onto the plane of the embeddings of the input sentences $A$ and $B$) and the embedding of sentence $B$. We normalize this angle such that the angle between the embeddings of sentences $A$ and $B$ is consistently 1. For computing the embedding we use \textbf{SBERT-L} and the results for other encoders are shown in the appendix.}
    \label{fig:mpnet_projection}
    % \vspace{-1mm}
\end{figure*}

==> Images_Codes/Model_Projection_Codes/olmo_projection.tex <==
\begin{figure*}[!t]
    % \vspace{-1mm}
    \centering

    % Overlap
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=1.0\textwidth]{Images/H2_Intersection/olmo_int.svg}
         \caption{TextOverlap: The projection embedding mostly lie in the ``middle'' of the embeddings of the input sentences as described in rubric R2 \ref{para:h2_results}.
         This follows  our expectation shown in figure \ref{fig:projection_expectation}b.
         }
         \label{fig:olmo_overlap}
     \end{subfigure}
     % \hfill
    ~
     % Difference
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
        \includesvg[width=1.0\textwidth]{Images/H5_Difference/olmo_diff.svg}
         \caption{TextDifference: The projection embedding is mostly bounded by a small angle around the embedding of the input sentence $A$ (refer R5 \ref{para:h5_results}).
         This follows  our expectation shown in figure \ref{fig:projection_expectation}a.
         }
         \label{fig:olmo_difference}
     \end{subfigure}
     % \hfill
    ~
    % Union
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=\textwidth]{Images/H6_Union/olmo_union.svg}
         \caption{
         TextUnion: The projection embedding mostly lie in ``middle'' of the input sentence embeddings (refer \ref{para:h6_results}). This follows  our expectation shown in figure \ref{fig:projection_expectation}c-middle. \\ \hspace{\textwidth}  
         }
         \label{fig:olmo_union}
     \end{subfigure}
     % \hfill
     

    \vspace{-1mm}
    \caption{Histogram of the angle between the projection of the overlap embedding (onto the plane of the embeddings of the input sentences $A$ and $B$) and the embedding of sentence $B$. We normalize this angle such that the angle between the embeddings of sentences $A$ and $B$ is consistently 1. For computing the embedding we use \textbf{OLMo} and the results for other encoders are shown in the appendix.}
    \label{fig:olmo_projection}
    % \vspace{-1mm}
\end{figure*}

==> Images_Codes/Model_Projection_Codes/openelm_projection.tex <==
\begin{figure*}[!t]
    % \vspace{-1mm}
    \centering

    % Overlap
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=1.0\textwidth]{Images/H2_Intersection/openelm_int.svg}
         \caption{TextOverlap: The projection embedding mostly lie in the ``middle'' of the embeddings of the input sentences as described in rubric R2 \ref{para:h2_results}.
         This follows  our expectation shown in figure \ref{fig:projection_expectation}b.
         }
         \label{fig:openelm_overlap}
     \end{subfigure}
     % \hfill
    ~
     % Difference
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
        \includesvg[width=1.0\textwidth]{Images/H5_Difference/openelm_diff.svg}
         \caption{TextDifference: The projection embedding is mostly bounded by a small angle around the embedding of the input sentence $A$ (refer R5 \ref{para:h5_results}).
         This follows  our expectation shown in figure \ref{fig:projection_expectation}a.
         }
         \label{fig:openelm_difference}
     \end{subfigure}
     % \hfill
    ~
    % Union
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=\textwidth]{Images/H6_Union/openelm_union.svg}
         \caption{
         TextUnion: The projection embedding mostly lie in ``middle'' of the input sentence embeddings (refer \ref{para:h6_results}). This follows  our expectation shown in figure \ref{fig:projection_expectation}c-middle. \\ \hspace{\textwidth}  
         }
         \label{fig:openelm_union}
     \end{subfigure}
     % \hfill
     

    \vspace{-1mm}
    \caption{Histogram of the angle between the projection of the overlap embedding (onto the plane of the embeddings of the input sentences $A$ and $B$) and the embedding of sentence $B$. We normalize this angle such that the angle between the embeddings of sentences $A$ and $B$ is consistently 1. For computing the embedding we use \textbf{OpenELM} and the results for other encoders are shown in the appendix.}
    \label{fig:openelm_projection}
    % \vspace{-1mm}
\end{figure*}

==> Images_Codes/Model_Projection_Codes/roberta_projection.tex <==
\begin{figure*}[!t]
    % \vspace{-1mm}
    \centering

    \begin{adjustbox}{width=1.0\textwidth}
    % Overlap
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=1.0\textwidth]{Images/H2_Intersection/roberta_int.svg}
         \caption{TextOverlap: The projection embedding mostly lie in the ``middle'' of the embeddings of the input sentences as described in rubric R2 \ref{para:h2_results}.
         This follows  our expectation shown in figure \ref{fig:projection_expectation}b.
         }
         \label{fig:roberta_overlap}
     \end{subfigure}
     % \hfill
    ~
     % Difference
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
        \includesvg[width=1.0\textwidth]{Images/H5_Difference/roberta_diff.svg}
         \caption{TextDifference: The projection embedding is mostly bounded by a small angle around the embedding of the input sentence $A$ (refer R5 \ref{para:h5_results}).
         This follows  our expectation shown in figure \ref{fig:projection_expectation}a.
         }
         \label{fig:roberta_difference}
     \end{subfigure}
     % \hfill
    ~
    % Union
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=1.0\textwidth]{Images/H6_Union/roberta_union.svg}
         \caption{
         TextUnion: The projection embedding mostly lie in ``middle'' of the input sentence embeddings (refer \ref{para:h6_results}). This follows  our expectation shown in figure \ref{fig:projection_expectation}c-middle. \\ \hspace{\textwidth} 
         }
         \label{fig:roberta_union}
     \end{subfigure}
     \end{adjustbox}
     % \hfill
     

    \vspace{-1mm}
    \caption{Histogram of the angle between the projection of the overlap embedding (onto the plane of the embeddings of the input sentences $A$ and $B$) and the embedding of sentence $B$. We normalize this angle such that the angle between the embeddings of sentences $A$ and $B$ is consistently 1. For computing the embedding we use \textbf{RoBERTa} and the results for other encoders are shown in the appendix.}
    \label{fig:roberta_projection}
    % \vspace{-1mm}
\end{figure*}

==> Images_Codes/Model_Projection_Codes/sbert_projection.tex <==
\begin{figure*}[!t]
    % \vspace{-1mm}
    \centering

    % Overlap
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=1.0\textwidth]{Images/H2_Intersection/sbert_int.svg}
         \caption{TextOverlap: The projection embedding mostly lie in the ``middle'' of the embeddings of the input sentences as described in rubric R2 \ref{para:h2_results}.
         This follows  our expectation shown in figure \ref{fig:projection_expectation}b.
         }
         \label{fig:sbert_overlap}
     \end{subfigure}
     % \hfill
    ~
     % Difference
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
        \includesvg[width=1.0\textwidth]{Images/H5_Difference/sbert_diff.svg}
         \caption{TextDifference: The projection embedding is mostly bounded by a small angle around the embedding of the input sentence $A$ (refer R5 \ref{para:h5_results}).
         This follows  our expectation shown in figure \ref{fig:projection_expectation}a.
         }
         \label{fig:sbert_difference}
     \end{subfigure}
     % \hfill
    ~
    % Union
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=1.0\textwidth]{Images/H6_Union/sbert_union.svg}
         \caption{
         TextUnion: The projection embedding mostly lie in ``middle'' of the input sentence embeddings (refer \ref{para:h6_results}). This follows  our expectation shown in figure \ref{fig:projection_expectation}c-middle. \\ \hspace{\textwidth} 
         }
         \label{fig:sbert_union}
     \end{subfigure}
     % \hfill
     

    \vspace{-1mm}
    \caption{Histogram of the angle between the projection of the overlap embedding (onto the plane of the embeddings of the input sentences $A$ and $B$) and the embedding of sentence $B$. We normalize this angle such that the angle between the embeddings of sentences $A$ and $B$ is consistently 1. For computing the embedding we use \textbf{SBERT-mini} and the results for other encoders are shown in the appendix.}
    \label{fig:sbert_projection}
    % \vspace{-1mm}
\end{figure*}

==> Images_Codes/Model_Projection_Codes/simcse_projection.tex <==
\begin{figure*}[!t]
    % \vspace{-1mm}
    \centering

    % Overlap
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=1.0\textwidth]{Images/H2_Intersection/simcse_int.svg}
         \caption{TextOverlap: The projection embedding mostly lie in the ``middle'' of the embeddings of the input sentences as described in rubric R2 \ref{para:h2_results}.
         This follows  our expectation shown in figure \ref{fig:projection_expectation}b.
         }
         \label{fig:simcse_overlap}
     \end{subfigure}
     % \hfill
    ~
     % Difference
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
        \includesvg[width=1.0\textwidth]{Images/H5_Difference/simcse_diff.svg}
         \caption{TextDifference: The projection embedding is mostly bounded by a small angle around the embedding of the input sentence $A$ (refer R5 \ref{para:h5_results}).
         This follows  our expectation shown in figure \ref{fig:projection_expectation}a.
         }
         \label{fig:simcse_difference}
     \end{subfigure}
     % \hfill
    ~
    % Union
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=1.0\textwidth]{Images/H6_Union/simcse_union.svg}
         \caption{
         TextUnion: The projection embedding mostly lie in ``middle'' of the input sentence embeddings (refer \ref{para:h6_results}). This follows  our expectation shown in figure \ref{fig:projection_expectation}c-middle. \\ \hspace{\textwidth} 
         }
         \label{fig:simcse_union}
     \end{subfigure}
     % \hfill
     

    \vspace{-1mm}
    \caption{Histogram of the angle between the projection of the overlap embedding (onto the plane of the embeddings of the input sentences $A$ and $B$) and the embedding of sentence $B$. We normalize this angle such that the angle between the embeddings of sentences $A$ and $B$ is consistently 1. For computing the embedding we use \textbf{SimCSE} and the results for other encoders are shown in the appendix.}
    \label{fig:simcse_projection}
    % \vspace{-1mm}
\end{figure*}

==> Images_Codes/Model_Projection_Codes/use_projection.tex <==
\begin{figure*}[!t]
    % \vspace{-1mm}
    \centering

    % Overlap
    \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=1.0\textwidth]{Images/H2_Intersection/use_int.svg}
         \caption{TextOverlap: The projection embedding mostly lie in the ``middle'' of the embeddings of the input sentences as described in rubric R2 \ref{para:h2_results}.
         This follows  our expectation shown in figure \ref{fig:projection_expectation}b.
         }
         \label{fig:use_overlap}
     \end{subfigure}
     % \hfill
    ~
     % Difference
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
        \includesvg[width=1.0\textwidth]{Images/H5_Difference/use_diff.svg}
         \caption{TextDifference: The projection embedding is mostly bounded by a small angle around the embedding of the input sentence $A$ (refer R5 \ref{para:h5_results}).
         This follows  our expectation shown in figure \ref{fig:projection_expectation}a.
         }
         \label{fig:use_difference}
     \end{subfigure}
     % \hfill
    ~
    % Union
     \begin{subfigure}[b]{0.3\textwidth}
         \centering
         \includesvg[width=\textwidth]{Images/H6_Union/use_union.svg}
         \caption{
         TextUnion: The projection embedding mostly lie in ``middle'' of the input sentence embeddings (refer \ref{para:h6_results}). This follows  our expectation shown in figure \ref{fig:projection_expectation}c-middle.  \\ \hspace{\textwidth}
         }
         \label{fig:use_union}
     \end{subfigure}
     % \hfill
     

    \vspace{-1mm}
    \caption{Histogram of the angle between the projection of the overlap embedding (onto the plane of the embeddings of the input sentences $A$ and $B$) and the embedding of sentence $B$. We normalize this angle such that the angle between the embeddings of sentences $A$ and $B$ is consistently 1. For computing the embedding we use \textbf{USE} and the results for other encoders are shown in the appendix. 
    }
    \label{fig:use_projection}
    % \vspace{-1mm}
\end{figure*}

==> Tables/dataset_examples.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Dataset Examples
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[!htb]%\small
\centering
\ra{1.0}

% Text Difference
\begin{subtable}[h]{1.0\textwidth}
    \centering
    \adjustbox{max width=\textwidth}{%
    \begin{tabular}{C{2.25cm}|C{2.25cm} | C{3cm}|C{3cm}|C{2.25cm}|C{2.25cm}}
        \toprule
         
         %%%%%%%%%%%%%%%%%%%%%%%%
         % % TextDifference %
         \multicolumn{6}{c}{\textbf{TextDifference}} \\


        %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
         % S2 perspective
         %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
         % Type I
         \midrule
         \multicolumn{2}{c|}{$\bm{A}$  $\bm{(S_{2})}$} &  \multicolumn{2}{c|}{$\bm{B}$  $\bm{(S_{curr})}$} & \multicolumn{2}{c}{$\bm{D}$  $\bm{(S_{next})}$} \\
         \midrule
         \multicolumn{2}{C{4.5cm}|}{``Congress sent legislation to fund veterans care at requested levels through Dec. 14, despite current funding still being below the \$3.9B passed, said Pelosi's spokesman.''} &  \multicolumn{2}{C{6cm}|}{``Congress also sent to the president legislation that would fund veterans care at the levels requested by the president through December 14, the leadership said.''} & \multicolumn{2}{C{4.5cm}}{``The current funding level "is still below the \$3.9 billion extra that we passed," said Nadeam Elshami, spokesman Pelosi.''} \\
         % Type II
         \midrule
         \multicolumn{2}{c|}{$\bm{A}$  $\bm{(S_{2})}$} &  \multicolumn{2}{c|}{$\bm{B}$  $\bm{(S_{next})}$} & \multicolumn{2}{c}{$\bm{D}$  $\bm{(S_{curr})}$} \\
         \midrule
         \multicolumn{2}{C{4.5cm}|}{``Congress sent legislation to fund veterans care at requested levels through Dec. 14, despite current funding still being below the \$3.9B passed, said Pelosi's spokesman.''} &  \multicolumn{2}{C{6cm}|}{``The current funding level "is still below the \$3.9 billion extra that we passed," said Nadeam Elshami, spokesman Pelosi.''} & \multicolumn{2}{C{4.5cm}}{``Congress also sent to the president legislation that would fund veterans care at the levels requested by the president through December 14, the leadership said.''} \\
         % Type III
         \midrule
         \multicolumn{2}{c|}{$\bm{A}$  $\bm{(S_{2})}$} &  \multicolumn{2}{c|}{$\bm{B}$  $\bm{(S_{1})}$} & \multicolumn{2}{c}{$\bm{D}$  $\bm{(S_{next})}$} \\
         \midrule
         \multicolumn{2}{C{4.5cm}|}{``Congress sent legislation to fund veterans care at requested levels through Dec. 14, despite current funding still being below the \$3.9B passed, said Pelosi's spokesman.''} &  \multicolumn{2}{C{6cm}|}{``According to the leadership, last year's Republican-controlled Congress never passed a separate bill funding veterans programs but sent a legislation funding veterans care to the president until December 14.''} & \multicolumn{2}{C{4.5cm}}{``The current funding level "is still below the \$3.9 billion extra that we passed," said Nadeam Elshami, spokesman Pelosi.''} \\
         
        \bottomrule
    \end{tabular}
    }
\end{subtable}

\caption{This table shows the synthetic sample for the \textit{TextUnion} operator using the sentences ($S_{curr}$, $S_{next}$, $S_1$ and $S_2$) mentioned in table \ref{tab:qualitative_input_samples}.
Here $A$ and $B$ corresponds to the input sentences and $D$ corresponds to the target ``difference'' sentence. 
More samples for TextDifference are shown in table \ref{tab:qualitative_difference1}. 
Follow section \ref{sec:dataset} for more details.}
\label{tab:dataset_examples}
\end{table*}

==> Tables/dataset_quantitative.tex <==
\begin{table}[!t]\footnotesize
    \centering
    \ra{1.0}
    \begin{adjustbox}{width=0.8\columnwidth}
    \begin{tabular}{c|c|c|c}
        \toprule
        % \multirow{2}{*}{\textbf{TextOverlap}} & \multirow{2}{*}{\textbf{TextDifference}} & \multirow{2}{*}{\textbf{TextUnion}} & 
        % \textbf{Overall} \\
        % & & &  \textbf{Average} \\

        \textbf{Text-} & \textbf{Text-} & \textbf{Text-} & \textbf{Overall} \\
        \textbf{Overlap} & \textbf{Difference} & \textbf{Union} & \textbf{Average} \\
        
        \midrule
        \midrule
        \multicolumn{4}{c}{\textbf{Average Annotation Score}} \\
        \midrule
        $2.51$ & $2.99$ & $2.81$ & $2.77$ \\
        % \midrule
        % \multicolumn{4}{c}{} \\ % Empty Line
        \midrule
        \multicolumn{4}{c}{
        \textbf{Satisfactory Samples Count (in $\mathbf{\%}$)}} \\ 
        \midrule
        $86.25$ & $95.75$ & $92$ & $91.33$ \\
        \bottomrule
    \end{tabular}
    \end{adjustbox}
    % \vspace{-1mm}
    \caption{
    Human evaluation scores of synthetic samples, averaged over $400$ samples per operator and $2$-$3$ annotators per sample, rated on a Likert scale from $0$ to $4$. 
    Each operator's average annotation score is $> 2.5$ and,
    overall, $> 90\%$ of the samples are deemed ``satisfactory'', with an average annotation score of $\ge 1.5$. 
    These results validate the efficacy of our methodology for generating synthetic samples as described in Section \ref{sec:dataset}.
    % Mean human evaluation scores (averaged over 400 samples per operator and 2-3 annotators per sample) of the synthetic samples, rated on a scale from 0 to 4.
    % The average score for samples associated with each operator $> 2.5$ , thereby validating the efficacy of our methodology for generating synthetic samples as described in Section \ref{sec:dataset}. Furthermore, the percentage are samples that are ``satisfactory'' i.e. having an average rating of $\ge 1.5$ are $> 90 \%$ on average across all the operators. 
    }
    \label{tab:quantitative_analysis}
    % \vspace{-2mm}
\end{table}


% \begin{table}[!t]\small
%     \centering
%     \ra{1.0}
%     \begin{tabular}{rc}
%         \toprule
%         \textbf{TextOverlap} & $2.51$ \\
%         \textbf{TextDifference} & $2.99$ \\
%         \textbf{TextUnion} & $2.81$ \\
%         \midrule
%         \textbf{Average} & $2.77$ \\
%         \bottomrule
%     \end{tabular}
%     \caption{
%     Mean human evaluation scores (averaged over 400 samples per operator and 2-3 annotators per sample) of the synthetic samples, rated on a scale from 0 to 4.
%     The average score for samples associated with each operator $\ge 2.5$ , thereby validating the efficacy of our methodology for generating synthetic samples as described in Section \ref{sec:dataset}.
%     }
%     \label{tab:quantitative_analysis}
% \end{table}

==> Tables/h1_analysis_average.tex <==
\begin{table}[!t]%\notsotiny
    \centering
    \ra{1.0}

    % Cos
    \begin{adjustbox}{width=0.9\columnwidth}
    % \begin{subtable}[h]{1.0\columnwidth}
    % \centering
    \begin{tabular}{rccc}
        \toprule
        \multirow{2}{*}{\textbf{Models}}
         & \multirow{2}{*}{Cos($A$, $B$)} & Cos($A$, $O$) $-$  & Cos($B$, $O$) $-$ \\
         & & Cos($A$, $B$) & Cos($A$, $B$) \\
         
        \midrule
        SBERT-mini & $0.5896$ & $0.0478$ & $0.1109$ \\
        LASER & $0.7433$ & $\color{red} -0.0019$ & $0.0171$ \\
        USE & $0.5406$ & $0.0417$ & $0.0886$ \\
        RoBERTa & $0.9859$ & $\color{red} -0.0005$ & $0.0011$ \\
        SBERT-L & $0.6082$ & $0.0471$ & $0.1023$ \\
        SimCSE & $0.7109$ & $0.0298$ & $0.0646$ \\
        InferSent & $0.8114$ & $0.0037$ & $0.0174$ \\
        \midrule
        GPT3 & $0.8909$ & $0.0125$ & $0.0253$ \\
        LLaMA2 & $0.8168$ & $\color{red} -0.0036$ & $0.0207$ \\
        Mistral & $0.823$ & $\color{red} -0.0007$ & $0.026$ \\
        LLaMA3 & $0.8055$ & $\color{red} -0.0088$ & $0.0204$ \\
        OLMo & $0.7525$ & $0.0015$ & $0.0367$ \\
        OpenELM & $0.9129$ & $\color{red} -0.0086$ & $0.0036$ \\
        LLaMA3.2 & $0.8776$ & $\color{red} -0.0017$ & $0.0166$ \\
        Qwen & $0.9411$ & $\color{red} -0.002$ & $0.0064$ \\
        Gemma & $0.7654$ & $\color{red} -0.0081$ & $0.0258$ \\
        \bottomrule
    \end{tabular}
    % \caption{Cosine similarity scores }
    % \label{subtab:h1_average_cos}
    % \end{subtable}
    \end{adjustbox}

    % \hfill
    % \newline

    % % NED Scores
    % \begin{subtable}[h]{1.0\columnwidth}
    % \centering
    % \begin{tabular}{rccc}
    %     \toprule
    %     \multirow{2}{*}{\textbf{Model}}
    %      & \multirow{2}{*}{NED($A$, $B$)} & NED($A$, $O$) $-$  & NED($B$, $O$) $-$ \\
    %      & & NED($A$, $B$) & NED($A$, $B$) \\
    %     \midrule
    %     SBERT & $0.205$ & $-0.024$ & $-0.055$ \\
    %     LASER & $0.233$ & $-0.006$ & $-0.023$ \\
    %     USE & $0.230$ & $-0.021$ & $-0.045$ \\
    %     RoBERTa & $0.0073$ &\color{red} $0.0003$ & $ -0.0006$ \\
    %     MPNet & $0.1959$ & $ -0.0235$ & $ -0.0512$ \\
    %     SimCSE & $0.1453$ & $-0.0149$ & $-0.0324$ \\
    %     InferSent & $0.1952$ & $-0.009$ & $-0.0235$ \\
    %     \midrule
    %     GPT3 & $0.055$ & $-0.007$ & $-0.013$ \\
    %     Llama2 & $0.094$ & $\color{red} 0.002$ & $-0.011$ \\
    %     Mistral & $0.0913$ & $0.0004$ & $-0.0133$ \\
    %     LLaMA3 & $0.0982$ & $0.0044$ & $-0.0102$ \\
    %     Olmo & $0.1253$ & $-0.0006$ & $-0.0183$ \\
    %     OpenELM & $0.0464$ & $0.0046$ & $-0.0019$ \\
        
    %     \bottomrule
    % \end{tabular}
    % \caption{Normalized Euclidean Distance (NED) Scores}
    % \label{subtab:h1_average_ned}
    % \end{subtable}

    % \vspace{-1mm}
    \caption{
    Pairwise Differences in average cosine similarity among $(A, B)$, $(A, O)$ and $(B, O)$, denoted as $Cos(A, O) - Cos(A, B)$ and $Cos(B, O) - Cos(A, B)$ where positive differences are desirable.
    % Positive differences are desired for similarity measures, while negative differences indicate favorable outcomes for distance measures. 
    Cases where the criteria are not met are marked in \textcolor{red}{red}. For details, refer to Section \ref{para:h1_results}.
    }
    \vspace{-3mm}
    \label{tab:h1_analysis_average}
\end{table}

==> Tables/h1_analysis_mean_std.tex <==
\begin{table*}[!t]%\notsotiny
    \centering
    \ra{1.0}

    % Cos
    % \begin{adjustbox}{width=1.0\columnwidth}
    % \begin{subtable}[h]{1.0\columnwidth}
    % \centering
    \begin{tabular}{rcc}
        \toprule
        \multirow{2}{*}{\textbf{Models}}
         & Cos($A$, $O$) $-$  & Cos($B$, $O$) $-$ \\
         & Cos($A$, $B$) & Cos($A$, $B$) \\
         
        \midrule
        SBERT-mini & $0.0478 \pm 0.127$ & $0.1109 \pm 0.1471 $ \\
        LASER & $-0.0019 \pm 0.0601$ & $0.0171 \pm 0.0679 $ \\
        USE & $0.0417 \pm 0.1168$ & $0.0886 \pm 0.1336 $ \\
        RoBERTa  & $-0.0005 \pm 0.0053$ & $0.0011 \pm 0.0058 $ \\
        SBERT-L & $0.0471 \pm 0.1237$ & $0.1023 \pm 0.1423 $ \\
        SimCSE & $0.0298 \pm 0.0899$ & $0.0646 \pm 0.1014$ \\
        InferSent & $0.0037 \pm 0.047$ & $0.0174 \pm 0.0523$ \\
        \midrule
        GPT3 & $0.0125 \pm 0.0291$ & $0.0253 \pm 0.0333 $ \\
        LLaMA2 & $-0.0036 \pm 0.0715$ & $0.0207 \pm 0.0783 $ \\
        Mistral & $-0.0007 \pm 0.0637$ & $0.026 \pm 0.0716$ \\
        LLaMA3 & $-0.0088 \pm 0.0718$ & $0.0204 \pm 0.0817$ \\
        OLMo & $0.0015 \pm 0.0787$ & $0.0367 \pm 0.0904$ \\
        OpenELM & $-0.0086 \pm 0.0715$ & $0.0036 \pm 0.0744$ \\
        LLaMA3.2 & $-0.0017 \pm 0.043$ & $0.0166 \pm 0.0488$ \\
        Qwen & $-0.002 \pm 0.0297$ & $0.0064 \pm 0.0322$ \\
        Gemma & $-0.0081 \pm 0.0774$ & $0.0258 \pm 0.09$ \\
        \bottomrule
    \end{tabular}
    % \caption{Cosine similarity scores }
    % \label{subtab:h1_average_cos}
    % \end{subtable}
    % \end{adjustbox}

    % \hfill
    % \newline

    % % NED Scores
    % \begin{subtable}[h]{1.0\columnwidth}
    % \centering
    % \begin{tabular}{rccc}
    %     \toprule
    %     \multirow{2}{*}{\textbf{Model}}
    %      & \multirow{2}{*}{NED($A$, $B$)} & NED($A$, $O$) $-$  & NED($B$, $O$) $-$ \\
    %      & & NED($A$, $B$) & NED($A$, $B$) \\
    %     \midrule
    %     SBERT & $0.205$ & $-0.024$ & $-0.055$ \\
    %     LASER & $0.233$ & $-0.006$ & $-0.023$ \\
    %     USE & $0.230$ & $-0.021$ & $-0.045$ \\
    %     RoBERTa & $0.0073$ &\color{red} $0.0003$ & $ -0.0006$ \\
    %     MPNet & $0.1959$ & $ -0.0235$ & $ -0.0512$ \\
    %     SimCSE & $0.1453$ & $-0.0149$ & $-0.0324$ \\
    %     InferSent & $0.1952$ & $-0.009$ & $-0.0235$ \\
    %     \midrule
    %     GPT3 & $0.055$ & $-0.007$ & $-0.013$ \\
    %     Llama2 & $0.094$ & $\color{red} 0.002$ & $-0.011$ \\
    %     Mistral & $0.0913$ & $0.0004$ & $-0.0133$ \\
    %     LLaMA3 & $0.0982$ & $0.0044$ & $-0.0102$ \\
    %     Olmo & $0.1253$ & $-0.0006$ & $-0.0183$ \\
    %     OpenELM & $0.0464$ & $0.0046$ & $-0.0019$ \\
        
    %     \bottomrule
    % \end{tabular}
    % \caption{Normalized Euclidean Distance (NED) Scores}
    % \label{subtab:h1_average_ned}
    % \end{subtable}

    % \vspace{-1mm}
    \caption{
    Mean Std
    }
    \vspace{-3mm}
    \label{tab:h1_analysis_mean_std}
\end{table*}

==> Tables/h3_analysis_average.tex <==
\begin{table}[!t]\notsotiny
    \centering
    \ra{1.0}

    % Cos
    \begin{subtable}[h]{1.0\columnwidth}
    \centering
    \begin{tabular}{rccc}
        \toprule
        \multirow{2}{*}{\textbf{Model}}
         & \multirow{2}{*}{Cos($B$, $D$)} & Cos($A$, $D$) $-$  & Cos($A$, $B$) $-$ \\
         & & Cos($B$, $D$) & Cos($B$, $D$) \\
         
        \midrule
        MiniLM-v2 & $0.1759$ & $0.4292$ & $0.4111$ \\
        LASER & $0.5787$ & $0.1535$ & $0.1547$ \\
        USE & $0.1718$ & $0.3825$ & $0.3678$ \\

        RoBERTa & $0.9706$ & $0.0137$ & $0.014$ \\
        MPNet-v2 & $0.2243$ & $0.4007$ & $0.3829$ \\
        SimCSE & $0.4202$ & $0.2966$ & $0.2872$ \\
        InferSent & $0.6954$ & $0.1105$ & $0.11$ \\

        \midrule
        
        GPT3 & $0.7871$ & $0.1093$ & $0.105$ \\
        LLaMA2 & $0.6618$ & $0.141$ & $0.1416$ \\
        Mistral & $0.6808$ & $0.1371$ & $0.1361$ \\
        LLaMA3 & $0.633$ & $0.1547$ & $0.1567$ \\
        OLMo & $0.5668$ & $0.1781$ & $0.1758$ \\
        OpenELM & $0.8193$ & $0.0807$ & $0.0835$ \\
        
        \bottomrule
    \end{tabular}
    % \caption{Cosine Similarity scores}
    \label{subtab:h3_average_cos}
    \end{subtable}

    \vspace{-0.8mm}
    % \hfill
    % \newline

    % % NED Scores
    % \begin{subtable}[h]{1.0\columnwidth}
    % \centering
    % \begin{tabular}{rccc}
    %     \toprule
    %     \multirow{2}{*}{\textbf{Model}}
    %      & \multirow{2}{*}{NED($B$, $D$)} & NED($A$, $D$) $-$  & NED($A$, $B$) $-$ \\
    %      & & NED($B$, $D$) & NED($B$, $D$) \\
    %     \midrule
    %     SBert & $0.412$ & $-0.215$ & $-0.206$ \\
    %     LASER & $0.359$ & $-0.126$ & $-0.124$ \\
    %     USE & $0.414$ & $-0.191$ & $-0.184$ \\
    %     \midrule
    %     GPT & $0.107$ & $-0.055$ & $-0.053$ \\
    %     Llama2 & $0.172$ & $-0.071$ & $-0.071$ \\
        
    %     \bottomrule
    % \end{tabular}
    % \caption{Normalized Euclidean Distance scores}
    % \label{subtab:h3_average_ned}
    % \end{subtable}

    \caption{
    Average cosine similarity scores for pairs $(B, D)$, $(A, D)$ and $(A, B)$ in terms of their pairwise differences, denoted as Cos$(A, D)$ $-$ Cos$(B, D)$ and Cos$(A, B)$  $-$ Cos$(B, D)$ where $Cos$ represents the similarity/distance measure.
    Positive differences are desired. 
    % Cases where the criteria are not met are highlighted in \textcolor{red}{red}.
    Results for other similarity and distance measures are shown in appendix table \ref{tab:h3_analysis_average_appendix}.
    }
    \label{tab:h3_analysis_average}
\end{table}

==> Tables/h4_analysis_average.tex <==
\begin{table}[!t]\small
    \centering
    \ra{1.0}
    \begin{tabular}{rcccc}
        \toprule
        \textbf{Model} & \textbf{Cosine} & \textbf{L1} & \textbf{L2} & \textbf{NED} \\
        \midrule
        SBert & $99.980$ & $99.969$ & $99.980$ & $99.980$ \\
        LASER & $99.999$ & $99.372$ & $99.901$ & $99.999$ \\
        USE & $99.992$ & $99.995$ & $99.992$ & $99.992$ \\
        \midrule
        GPT & $99.991$ & $99.987$ & $99.991$ & $99.991$ \\
        Llama2 & $99.910$ & $93.122$ & $92.633$ & $99.914$ \\
        
        
        \bottomrule
    \end{tabular}
    \caption{H4 Analysis Average}
    \label{tab:h4_analysis_average}
\end{table}
